3D$^2$-Actor: Learning Pose-Conditioned 3D-Aware Denoiser for Realistic Gaussian Avatar Modeling

Advancements in neural implicit representations and differentiable rendering have markedly improved the ability to learn animatable 3D avatars from sparse multi-view RGB videos. However, current methods that map observation space to canonical space often face challenges in capturing pose-dependent details and generalizing to novel poses. While diffusion models have demonstrated remarkable zero-shot capabilities in 2D image generation, their potential for creating animatable 3D avatars from 2D inputs remains underexplored. In this work, we introduce 3D$^2$-Actor, a novel approach featuring a pose-conditioned 3D-aware human modeling pipeline that integrates iterative 2D denoising and 3D rectifying steps. The 2D denoiser, guided by pose cues, generates detailed multi-view images that provide the rich feature set necessary for high-fidelity 3D reconstruction and pose rendering. Complementing this, our Gaussian-based 3D rectifier renders images with enhanced 3D consistency through a two-stage projection strategy and a novel local coordinate representation. Additionally, we propose an innovative sampling strategy to ensure smooth temporal continuity across frames in video synthesis. Our method effectively addresses the limitations of traditional numerical solutions in handling ill-posed mappings, producing realistic and animatable 3D human avatars. Experimental results demonstrate that 3D$^2$-Actor excels in high-fidelity avatar modeling and robustly generalizes to novel poses. Code is available at: https://github.com/silence-tang/GaussianActor.

==> tables/abl_local_coord.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{}}
    \toprule
    
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{313}  & \multicolumn{3}{c}{315}
    
    \\ \cmidrule(l){2-7}
    & {\textcolor{mygray}{\fontsize{9pt}{9pt}\selectfont PSNR$\uparrow$}} & {\fontsize{9pt}{9pt}\selectfont LPIPS$\downarrow$} & {\fontsize{9pt}{9pt}\selectfont FID$\downarrow$} & {\textcolor{mygray}{\fontsize{9pt}{9pt}\selectfont PSNR$\uparrow$}} & {\fontsize{9pt}{9pt}\selectfont LPIPS$\downarrow$} & {\fontsize{9pt}{9pt}\selectfont FID$\downarrow$}
    
    \\ \midrule
    
    Ours w/o glc. & \textcolor{mygray}{\fontsize{9pt}{9pt}\selectfont 22.7} & \fontsize{9pt}{9pt}\selectfont 0.091 & \fontsize{9pt}{9pt}\selectfont 24.5 & \textcolor{mygray}{\fontsize{9pt}{9pt}\selectfont 20.0} & {\fontsize{9pt}{9pt}\selectfont 0.102} & \fontsize{9pt}{9pt}\selectfont 23.8 \\
    
    Ours w/ glc. & \textbf{\textcolor{mygray}{\fontsize{9pt}{9pt}\selectfont 23.5}} & {\textbf{\fontsize{9pt}{9pt}\selectfont 0.080}} & {\textbf{\fontsize{9pt}{9pt}\selectfont 19.6}} & \textbf{\textcolor{mygray}{\fontsize{9pt}{9pt}\selectfont 20.7}} & \textbf{\fontsize{9pt}{9pt}\selectfont 0.090} & {\textbf{\fontsize{9pt}{9pt}\selectfont 20.2}}
    \\ \midrule
    \end{tabular}
    \caption{Quantitative ablation study on the design of our Mesh-based Gaussian Local Coordinates. w/ and w/o glc denotes with and without Gaussian Local Coordinates, respectively.}
    \label{tab:abl_local_coord}
\end{table}

